Infrared and hard X-ray diagnostics of AGN identification from the Swift/BAT and AKARI all-sky surveys

We combine data from two all-sky surveys in order to study the connection between the infrared and hard X-ray (>10keV) properties for local active galactic nuclei (AGN). The Swift/Burst Alert Telescope all-sky survey provides an unbiased, flux-limited selection of hard X-ray detected AGN. Cross-correlating the 22-month hard X-ray survey with the AKARI all-sky survey, we studied 158 AGN detected by the AKARI instruments. We find a strong correlation for most AGN between the infrared (9, 18, and 90 micron) and hard X-ray (14-195 keV) luminosities, and quantify the correlation for various subsamples of AGN. Partial correlation analysis confirms the intrinsic correlation after removing the redshift contribution. The correlation for radio galaxies has a slope and normalization identical to that for Seyfert 1s, implying similar hard X-ray/infrared emission processes in both. In contrast, Compton-thick sources show a large deficit in the hard X-ray band, because high gas column densities diminish even their hard X-ray luminosities. We propose two photometric diagnostics for source classification: one is an X-ray luminosity vs. infrared color diagram, in which type 1 radio-loud AGN are well isolated from the others in the sample. The other uses the X-ray vs. infrared color as a useful redshift-independent indicator for identifying Compton-thick AGN. Importantly, Compton-thick AGN and starburst galaxies in composite systems can also be differentiated in this plane based upon their hard X-ray fluxes and dust temperatures. This diagram may be useful as a new indicator to classify objects in new and upcoming surveys such as WISE and NuSTAR.

==> figtex/FFplot.tex <==
\begin{figure}[!ht]
 \begin{minipage}{0.5\hsize}
  \begin{center}
   \includegraphics[width=65mm]{./fig/Result-111025-flux-ALL-111121.eps}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.5\hsize}
  \begin{center}
   \includegraphics[width=65mm]{./fig/flux18-fluxx-ALL-111025-111121.eps}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.5\hsize}
\vspace{5pt}
  \begin{center}
   \includegraphics[width=65mm]{./fig/flux90-fluxx-ALL-111025-111121.eps}
  \end{center}
 \end{minipage}
\caption{Flux-flux plot of the {\it AKARI} and {\it Swift}/BAT detected sources.
The vertical axes are hard X-ray fluxes (14 -- 195~keV). 
The horizontal axes are IR fluxes at (a) 9~$\mu$m, (b) 18~$\mu$m, and (c) 90~$\mu$m.
Each symbol describes AGN type (Seyfert~1, Seyfert~2, LINERs, and Blazars) taken from \cite{2010ApJS..186..378T}. 
Magenta characters ``C'' are Compton thick sources.}
\label{fig:FFplot}
\end{figure}
